FBMC Receiver Design and Analysis for Medium and Large Scale Antenna Systems

In this paper, we design receivers for filter bank multicarrier-based (FBMC-based) massive MIMO considering practical aspects such as channel estimation and equalization. In particular, we propose a spectrally efficient pilot structure and a channel estimation technique in the uplink to jointly estimate all the users' channel impulse responses. We mathematically analyze our proposed channel estimator and find the statistics of the channel estimation errors. These statistics are incorporated into our proposed equalizers to deal with the imperfect channel state information (CSI) effect. We revisit the channel equalization problem for FBMC-based massive MIMO, address the shortcomings of the existing equalizers in the literature, and make them more applicable to practical scenarios. The proposed receiver in this paper consists of two stages. In the first stage, a linear combining of the received signals at the base station (BS) antennas provides a coarse channel equalization and removes any multiuser interference. In the second stage, a per subcarrier fractionally spaced equalizer (FSE) takes care of any residual distortion of the channel for the user of interest. We propose an FSE design based on the equivalent channel at the linear combiner output. This enables the applicability of our proposed technique to small and/or distributed antenna setups such as cell-free massive MIMO. Finally, the efficacy of the proposed techniques is corroborated through numerical analysis.

==> cellfree_simulation.tex <==
 \subsection{FBMC Simulation Results}
 \label{sec:cellfresimulation}
 In this section, we evaluate our mathematical developments of cell-free FBMC massive-MIMO. We perform our simulation analysis based on a cell-free massive MIMO setup with APs that are located on a regular grid in a $2\times2$ square kilometers area. Each AP has $4$ antennas. We deploy the wrap-around technique \cite{bjornson2019making} to imitate the infinite area and avoid boundary effect. We consider $K=4$ users that take random locations in each realization. In our simulations for cell-free scenario, we consider same PDP as co-located setup scaled with large-scale fading coefficients. The large-scale fading coefficients are modeled employing the COST Hata model as \cite{damosso1999cost}
\be
10\text{log}_{10}(\beta_{i,k}) = -135-35\text{log}_{10}(d_{i,k})-\mathcal{X}_{i,k},
\ee \vspace{-1mm}
where $d_{i,k}$ is the distance between a given user $k$ and antenna $i$ in kilometers and $\mathcal{X}_{i,k} \sim \mathcal{CN}(0, \sigma^2_{\mathcal{X}})$  represents shadowing effect with $\sigma^2_{\mathcal{X}}=8$ dB. Variance of noise is calculated using the noise figure as $\sigma^2_{\eta} = \mathcal{K} \times \kappa_{\rm B} \times {\rm B} \times {\rm NF}$,
%\be
%\sigma^2_{\eta} = \mathcal{K} \times \kappa \times {\rm B} \times {\rm NF}
%\ee
where $\mathcal{K}$, $\kappa_{\rm B}$, $B$, and NF are temperature in kelvin, Boltzmann constant, bandwidth, and noise figure, respectively. In this part, we consider $\mathcal{K}=290$~K, $\kappa_{\rm B} = 1.3 \times 10^{-23}$~J/K, $B=20$~MHz and NF~$=9$ dB. The maximum transmit power of each user is assumed to be $200$~mW.


Fig. \ref{fig:cdf} illustrates the cumulative distribution function (CDF) of the signal-to-interference ratio (SIR) performance for FBMC- and OFDM-based cell-free MIMO having $9$ APs and $4$ users with and without power control, i.e., $\nu=0$ and $\nu=1$, respectively. This result shows that power control is beneficial to both waveforms as it will lead to an improved SIR performance and hence a higher quality of service. It is worth to note that SIR performance of FBMC in cell-free scenario is not reported before. This result shows, FBMC and OFDM have the same performance in terms of CDF. 
The values for fractionally power control appears in the range $[0.5, 0.7]$, such as \cite{muhammad2009performance,quintero2008advanced,nikbakht2020uplink}, with lower values favoring the average SIR while higher values promote fairness and cell-edge performance. Accordingly, we chose to perform our simulation with $\nu = 0.5$.

In the rest of the simulation results, we consider the fractional power control, i.e., $\nu=0.5$, as per \textcolor{red}{LTE} recommendation. 

\begin{figure}
		\centering
		\includegraphics[scale=0.625,trim={0 0 0 0},clip]{figures/CDF_OFDM_FBMC_4K.eps}
		\caption{The empirical CDF of OFDM and FBMC compared while using maximum power and power control.}
		\label{fig:cdf}
	\end{figure}
	
	\begin{figure}
		\centering
		\includegraphics[scale=0.595,trim={0 0 0 0},clip]{figures/CellFreeSINRperfect.eps}
		\caption{Output SINR vs. number of APs, $N_{AP}$, for FSE design  $L_{\rm FSE}=5$.}
		\label{fig:perfectCSI_cellfree_ZF}
	\end{figure}
	
In Fig.~\ref{fig:perfectCSI_cellfree_ZF}, the SINR of our proposed FSE design with the length $L_{\rm FSE}=5$ is compared with OFDM as a benchmark. We assumed channel estimates are perfect and ZF used for linear combining. As this figure shows, our proposed equivalent channel-based FSE achieves similar performance to OFDM. This result shows the effectiveness of our method in the case of cell-free with a wide range of large-scale fading alternations. For the larger antenna setup, the gap between FBMC and OFDM comes from a small length of FSE and can be mitigated using an equalizer with a higher length. 


	\begin{figure}
		\centering		\includegraphics[scale=0.6,trim={0 0 0 0},clip]{figures/CellFreeSINRimperfect.eps}
		\caption{Output SINR vs. number of APs, $N_{AP}$, for FSE design  $L_{\rm FSE}=5$.}
		\label{fig:cellfree_imperfectCSI}
\end{figure}

Fig.~\ref{fig:cellfree_imperfectCSI} depicts the efficacy of the proposed modified equalizers in Section~\ref{sec:imperfect}. The performance of the modified equalizer surpasses the equalizer with no compensation. Similar to co-located setup, in this case, as the number of APs increases, the compensation of channel estimate errors is more significant.




